Spin relaxation, Josephson effect and Yu-Shiba-Rusinov states in superconducting bilayer graphene

Bilayer graphene has two non-equivalent sublattices and, therefore, the same adatom impurity can manifest in spectrally distinct ways-sharp versus broad resonances near the charge neutrality-depending on the sublattice it adsorbs at. Employing Green's function analytical methods and the numerical Kwant package we investigate the spectral and transport interplay between the resonances and superconducting coherence induced in bilayer graphene by proximity to an s-wave superconductor. Analyzing doping and temperature dependencies of quasi-particle spin-relaxation rates, energies of Yu-Shiba-Rusinov states, Andreev spectra and the supercurrent characteristics of Josephson junctions we find unique superconducting signatures discriminating between resonant and off-resonant regimes. Our findings are in certain aspects going beyond the superconducting bilayer graphene and hold for generic s-wave superconductors functionalized by the resonant magnetic impurities.

==> latexmkrc <==
add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );

sub makeexternaldocument {
    if (!($root_filename eq $_[0]))
    {
        # FOR PDFLATEX
        system( "latexmk -cd -pdf \"$_[0]\"" );

        # FOR LATEX+DVIPDF
        # system( "latexmk -cd \"$_[0]\"" );

        # FOR XELATEX
        # system( "latexmk -cd -xelatex \"$_[0]\"" );
        
        # FOR LUALATEX
        # system( "latexmk -cd -lualatex \"$_[0]\"" );
   }
}

